Any Other Thoughts, Hedgehog? Linking Deliberation Chains in Collaborative Dialogues

Question-asking in collaborative dialogue has long been established as key to knowledge construction, both in internal and collaborative problem solving. In this work, we examine probing questions in collaborative dialogues: questions that explicitly elicit responses from the speaker's interlocutors. Specifically, we focus on modeling the causal relations that lead directly from utterances earlier in the dialogue to the emergence of the probing question. We model these relations using a novel graph-based framework of deliberation chains, and reframe the problem of constructing such chains as a coreference-style clustering problem. Our framework jointly models probing and causal utterances and the links between them, and we evaluate on two challenging collaborative task datasets: the Weights Task and DeliData. Our results demonstrate the effectiveness of our theoretically-grounded approach compared to both baselines and stronger coreference approaches, and establish a standard of performance in this novel task.

==> colored_deli_table.tex <==
\begin{table*}[!ht]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}lllrrrrrrrrrrrrrrrrr@{}}
            \toprule
            &&& \multicolumn{3}{c}{MUC} && \multicolumn{3}{c}{$B^3$} && \multicolumn{3}{c}{$CEAFe$} && CoNLL\\
            \cmidrule{4-6} \cmidrule{8-10} \cmidrule{12-14} \cmidrule{16-16}
            &&& R & P & $F_1$ && R & P & $F_1$ && R & P & $F_1$ && \multicolumn{1}{r}{$F_1$} \\ 
            \midrule
            & LLaMA 2-7B-chat && \cellcolor{yellow!50}\textbf{99.9} & 88.5 & \cellcolor{yellow!50}\textbf{93.8} && \cellcolor{yellow!50}\textbf{99.9} & 49.7 & 66.4 && 35.9 & \cellcolor{yellow!50}\textbf{77.1} & 49.0 && 69.7 \\
            & --- Ours (Joint + $W$) && 92.7 & \cellcolor{yellow!50}\textbf{91.5} & 90.9 && 92.3 & \cellcolor{yellow!50}\textbf{72.6} & \cellcolor{yellow!50}\textbf{79.5} && \cellcolor{yellow!50}\textbf{64.4} & 55.9 & \cellcolor{yellow!50}\textbf{59.9} && \cellcolor{yellow!50}\textbf{76.4} \\
            \bottomrule
        \end{tabular}
    }
    \caption{DeliData test set results. ``LongContext'' denotes \citet{caciularu2021cdlm}'s coreference methodology applied to deliberation chain clustering. ``Bidirectional'' denotes \citet{ahmed20232}'s methodology.}
    \label{tab:deli_colored_table}
\end{table*}

==> cosine_baseline.tex <==
\begin{table*}
\caption{Probing and Causal Counterpart Clustering Results on DeliData (Cosine Similarity)}
\label{tab:cosine_similarity_scores_deli}
\centering
\begin{tabular}{cccccccccccccc}
\toprule
Dataset & M R & M P & M F1 & B3 R & B3 P & B3 F1 & Cf R & Cf P & Cf F1 & LEA R & LEA P & LEA F1 & CoNLL F1 \\
\midrule

xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\ 
xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\ 

\bottomrule
\end{tabular}
\end{table*}

==> deli_full_table_results_dev.tex <==
\begin{table*}[!ht]
    \centering
     
 \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lllrrrrrrrrrrrrrrrrr@{}}
    \toprule
    &&& \multicolumn{3}{c}{MUC} && \multicolumn{3}{@{}c@{}}{$B^3$} & & \multicolumn{3}{c}{$CEAFe$} && CoNLL\\
    \cmidrule{4-6} \cmidrule{8-10} \cmidrule{12-14} \cmidrule{16-16}
    &&& R & P & $F_1$ && R & P & $F_1$ && R &P & $F_1$ && \multicolumn{1}{r}{$F_1$}  \\ 
   \midrule

        

         

      
       
        & LongContext (full previous history) && 89.7  & 89.6 & 89.7 && 88.3 & 64.1 & 74.3 && 52.6 & 52.9 & 52.7 && 72.2 \\
      & Bidirectional  && 96.8  & 90.3 & 93.4 && 96.6 & 59.4 & 73.5 && 48.1 & 70.9 & 57.3 && 74.7 \\
    
       & \textbf{Joint} (ours)  && 95.6  & 91.3 & 93.4 && 95.2 & 63.8 & 76.4 && 54.9 & 69.8 & 61.5 && 77.1 \\
       & Joint (dummy, w/o CC and PP) && 92.7  & 89.2 & 90.9 && 92.3 & 60.5 & 73.1 && 52.1 & 62.4 & 56.8 && 73.6  \\
      &LLaMA 2-7B-Chat (zero-shot)  && 84.2  & 76.3 & 80.1 && 82.7 & 73.2 & 77.7 && 67.5 & 77.2 & 72.0 && 76.6  \\
        
       & GPT-3.5-Turbo (zero-shot)  && 81.7  & 81.0 & 81.4 && 81.0 & 78.6 & 79.8 && 76.1 & 77.0 & 76.5 && 79.2 \\

       



      
    
       
% & $Long_\text{+ROEC,-KD}$ (ours) && 79.4  & \textbf{92.4} & 85.4 && 79.8 & \textbf{93.1} & 85.9 && \textbf{89.1} & 76.1 & 82.1 && 84.5 \\ 
%         & $Long_\text{-ROEC,+KD}$ (ours)  && 78.2  & 90.6 & 83.9 && 79.4 & 90.2 & 84.4 && 87.9 & 75.4 & 81.2 && 83.2 \\
%         &  $Long_\text{+ROEC,+KD}$ (ours) && 84.1  & 92.0 & 87.9 && 82.4 & 91.7 & \textbf{86.8} && 88.9 & 80.5 & \textbf{84.5} && \textbf{86.4} \\
 
 

    \bottomrule
    \end{tabular}}
    \caption{Delidata Dev Set full results}
    \label{tab:deli_full_results_dev}
\end{table*}


==> nath.tex <==
We carried out extensive evaluations to ensure that GPT-annotated causal interventions are coherent, 

—While carrying out our initial experiments we found that GPT 3.5 turbo generations typically tend to work best for an average of 25 utterances prior to the probing intervention. Since gold probing interventions are manually labelled in the Delidata corpus, we have access their sequential time steps in the utterance history. This allows us to accurately map GPT generations back to the actual causal interventions present. 

Therefore, to generate high-quality GPT causal interventions we first contextualized each instance of causal intervention generation/extraction on both the probing utterance as well as the previous utterance history \cite{ works that show how to contextualize GPT generations}. Secondly, since context history affects GPT performance non-trivially\cite{ GPT struggles with longer context length in dialogue generation etc) }and since the WTD dataset has longer dialogue sequences, we restricted our context window to 25 utterances for a probing question. 
This strategy has been applied \citeP{where?} (of context length overlapping instead  of using the entire history )and allows us to accurately generate causal responses for clustering.  In order to further validate the casual interventions, we carried out a human evaluation of the generated interventions on various axes of quality evaluation as well as inter-annotator agreement. 












\paragraph{Clarifying questions Vs Probing Questions?}

—clarifying questions are asked when there is some ambiguity or underspecification in a dialogue; OTOH, probing questions i.e. any utterance that provokes discussion, deliberation or argumentation \textit{without} introducing novel information. So why do we only model previous utterances in finding the causal counterparts: one, due to causality and by definition, probing questions should not introduce new topics/information not already present up until that state in the dialogue. 

—\textbf{most previous work has been about clarifying questions}; less work on probing utterances or questions. Moreover, as as we know, no previous work has investigates the causal points in a dialogue that gives rise to probing utterances. In contrast to clarifying questions that result from ambiguity or underspecification mostly from the immediate previous utterance, causal points resulting in probing questions can theoretically occur at any previous point in the discourse (

\paragraph{How does clustering causal utterances help in friction/deliberative reasoning generation in collaborative tasks?}

—this is the first step in ensuring that any friction generation component in an embodied collaborative task is grounded in a contextual understanding of the dialogue with specific focus on the causal utterances that forms the \textit{attentional state} in any linguistic act~\cite{grosz1986attention}. Detecting and clustering the causal origins of a deliberative utterance directly impacts LLM-agent oriented autoregressive generation of friction in the dialogue as it abstracts way specific causal utterances and model underlying causal relationships between them ( as in we can use these clusterings to not only model friction but also specifically ground/constrain the decoding/generation component \cite{hokamp-liu-2017-lexically, geng2024grammarconstrained, de2020autoregressive} to reflect causality in collaborative tasks)


—get negative rational pairs:
—get remaining keys 

—design the positive and negative pairs for training: 
—try the average of the three scores 
—then try the joint learning in a ranking framework 
—then try lemma baseline 
—and perhaps try long former 
—try the clustering pipeline after initial results 
—get results with the coref pipeline 



—joint learning framework:


—why do we need to cluster probing questions with causal counterparts?

-detecting the causal counterparts is a conditional problem since 

—theoretically, a causal delivery can prompt more than one questions but we find from an empirical verification of the dataset that 

—most previous work in dialogue modeling investigate how and when to generate clarifying questions but less work has been done on analyzing the nature of probing questions and Ling them with their casual counterparts..

—why is it a retrieval problem? Retrieval will help up 

—we define the conversational length limit of each probing question with its causal counterparts using discourse coherence theory and the “attention state” within a dialogue trajectory. This allows us to restrict the search space of casual counterparts to the previous utterances in the specific dialogue instance from the start of the dialogue. In practice though, we limit the previous candidate utterances to reflect the average number of 

—we e3xperimnent with the entire dialogue history in deidata since the average length of the dialogue in this case is considerably lower than weights task which contains much longer dialogues. For consistency, we restrict candidate generation to the average of the dialogue lengths in each dataset to reflect dataset characteristics. 



 Why is framing the causal counterpart retrieval problem as a coreference-resolution-based clustering problem helpful?

—in pairwise framework for encoding  probing utterance and its context for Ling the causal counterparts, thus contextual cues relevant for making that decision are explicitly modeled during the training stage and helps locate specific cues in the context that leads to a correct decision at inference. This allows a deep and thorough examination of cues embedded

—reduces search space: we don’t have to compute counterparts pairwise scores. Typically, each document has n 
—attentional state in a dialogue and interleaved discourses: 
—probing questions act as pivot: almost at an entity-level similar to a coreference world entity. 

—since transitivity is natural here ( each casual counterpart is causally related to one specific probing question or gives rise to one specific probing question so if A -> P and B-> P then A->B ) modeling probing questions with causal counterparts reduces the search space of the quadratic complexity of computing pairwise scores of causal pairs in pairwise comparisons, both at inference as well as in training. 









\paragraph{Inference}


\begin{equation}
\small
Pr(p_i = p \mid D) = \frac{\exp(\Phi_P(p, s_i))}{\sum_{p' \in \mathcal{L}_P} \exp(\Phi_P(p', s_i))}
\end{equation}

\begin{equation}
\small
Pr(c_i = c \mid D) = \frac{\exp(\Phi_C(c, s_i))}{\sum_{c' \in \mathcal{L}_C} \exp(\Phi_C(c', s_i))}
\end{equation}

\begin{equation}
\small
Pr(l_{ij} = l \mid D) = \frac{\exp(\Phi_{L}(l, s_i, s_j))}{\sum_{l' \in \mathcal{L}_{L}} \exp(\Phi_{L}(l', s_i, s_j))},
\end{equation}

where \(\Phi_P\) denotes the unnormalized model score for a probing intervention \( p \) and a span \( s_i \), \(\Phi_C\) denotes the score for a causal intervention \( c \) and a span \( s_i \), and \(\Phi_{L}\) denotes the score for a link \( l \) between \( p \) and \( c \) for span pairs \( s_i \) and \( s_j \). These \(\Phi\) scores are further decomposed into span and pairwise span scores computed from feed-forward networks.

%





% Since a probing intervention can "cause" or lead to another probing statement within a dialogue~\cite{sukmadewi2014improving, behr2012asking}, we do \texit{not}omit probing labels from the previous utterances given as context. Additionally, in the absence of ATOMIC-like KBs containing deliberative reasoning triples, we leverage COT-type reasoning by explicitly asking the LLM to generate free-text rationales (FTRs) with the probing intervention as the evidence. This establishes a one-to-one map between a probing intervention with its GPT-extracted causal interventions at the end of the loop. Such a strategy serves two crucial goals in validating the gold chains: 1) rationales can be used as additional reference during human evaluation to validate the GPT annotations and how aligned they are with human reasoning (See Appendix for human evaluation component) . 2) this iterative prompting strategy ensures that the annotated deliberation chains always start and end with a causal and probing intervention respectively at the end of the loop. 

% The above strategy however leads to cases where a single casual interventions are extracted for multiple probing. As such, our gold mapping algorithm thereafter iteratively assigns singular gold labels for these chains such that the deliberation graph remains connected. The algorithm finally outputs the gold intervention clusters that we evaluate our framework on. See Appendix for our detailed gold-label assignment algorithm and Table.\ref{tab:cluster_statistics_deli_wtd} for cluster level details of the two datasets.

% , starting at the initial index of a probing intervention within a dialogue. 



% More specifically, we augment contextual information like a set of X\footnote{We provide context of }previous utterances which acts as the target set of utterances for causal intervention extraction. 


% without a common knowledge-base (KB) like ATOMIC\cite{sap2019atomic} for deliberative "task-based" reasoning, we give gold labels of probing interventions. We iteratively prompt {\tt GPT-3.5-turbo-0125} to extract causal interventions for each probing intervention, starting at the initial index of a probing intervention within a dialogue. More specifically, we augment contextual information like a set of X\footnote{We provide context of }previous utterances which acts as the target set of utterances for causal intervention extraction. 




—connection between P and C and I and j as antecedents 
—need learning overall  probability 
—need scoring, like what are the scores?
--representations
Training: loss function ( P , C and L)






\an{\textbf{Definition 2.} Consider a deliberation graph \( G = (V, E_1, E_2, \lambda) \).  A \textbf{deliberation chain} \( G' \) or a \textit{intervention cluster\footnote{We use the term \textit{intervention cluster(s)} and \textit{deliberation cluster(s)} interchangeably to refer to the linked chain of a specific probing intervention with its causal interventions upon transitive closure. This is similar to how a entity cluster is defined in  coreference resolution literature.}} is a subgraph \( G' = (V', E'_1, E'_2, \lambda) \) of \( G \), such that \( \{\text{P}_{\hat i} , \text{C}_{\hat j} \} \subseteq V' \) , where \( \text{P}_{\hat i} = \min\{ i \mid \lambda(\text{P}_i) \in V \} \) and \( \text{C}_{\hat i}  = \min\{ j \mid \lambda(\text{C}_j) \in V \} \) indicate the initial occurrences in the traversal of \( G \) from causal to probing interventions.}


\textbf{Lemma 1: Disconnection via Transitive Closure.} From definition 2, let \( \mathcal{T}(E'_1) \) denote the transitive closure of \( E'_1 \). If \( \mathcal{T}(E'_1) \) induces a partition of \( V' \) into \( k \) disconnected components, then we can express this as \( \bigcup_{i=1}^{k} V'_i = V' \) and \( V'_i \cap V'_j = \emptyset \) for \( i \neq j \), resulting in \( G' \) becoming disconnected. Since our datasets contain not inter-cluster linkages (as in, a probing intervention can almost never have a causal counterpart in a separate dialogue group), our learning algorithm implicitly learns such trends from the data distribution. This ensures that it is sensitive to potential overclustering in disconnected \textit{gold} intervention clusters. 


% \an{\textbf{Lemma 1: Disconnection via Transitive Closure.} From Definition 2, let \( \mathcal{T}(\mathcal{E}'_1) \) denote the transitive closure of \( \mathcal{E}'_1 \). If \( \mathcal{T}(\mathcal{E}'_1) \) induces a partition of \( \mathcal{V}' \) into \( k \) disconnected components, then we can express this as \( \bigcup_{i=1}^{k} \mathcal{V}'_i = \mathcal{V}' \) and \( \mathcal{V}'_i \cap \mathcal{V}'_j = \emptyset \) for \( i \neq j \), resulting in \( \mathcal{G}' \) becoming disconnected. Since our datasets contain no inter-cluster linkages (i.e., a probing intervention cannot have a causal counterpart in a separate dialogue group), our learning algorithm implicitly learns such trends from the data distribution. This ensures that it is sensitive to potential overclustering in disconnected \textit{gold} intervention clusters.}

% \textbf{Lemma 2: Transitive Efficiency.} The application of transitive closure on \( E'_1 \) in \( G' \) requires fewer comparisons than pairwise connections in standard entity clustering~\cite{lee2012joint, cattan2021cross, held-etal-2021-focus}, due to the ordered structure of \( V' \).


% I have written down the pipeline with the refined causal counterpart (not sure if counterpart is the right word for it but I will check what else is an option). Currently, I am generating a set of counterparts (3) for each probing question (with participants name info and previous utterance history right before the probing statement) and for each counterpart, a rationale is also generated. I am only getting the them with gpt-3.5-turbo-0125 (latest model right under gpt4). Reviewers will surely ask about the quality of generations so we are also designing a way to verify them: I think 1) human evals of a subset 2) heuristic eval of the entire generations could be important proxies to evaluate the quality of the counterparts.  The heuristics can be of two types: a) some form of logical combination where a causal cp can only be a solution statement from a different participant (etc etc) and b) lemma based heuristic (cc statements typically contain a specific vowel or odd/even number that overlaps with similar info in the probing statement). This could be a section on the quality of the generations/annotations
% As for model design, I did some digging and it seems like one single end to end joint model might be feasible, otherwise we can always design a retrieve candidates with a bi-encoder adn score top-k with cross encoder. Joint learning might be more interesting though





Prelim results


\begin{table*}[ht]
    
 
\centering
 
     
 \footnotesize
\caption{Probing and Causal Counterpart Clustering Results on DeliData}
\label{tab:coref_metrics}
\begin{tabular}{cccccccccccccc}
\toprule
Epoch & M R & M P & M F1 & B3 R & B3 P & B3 F1 & Cf R & Cf P & Cf F1 & LEA R & LEA P & LEA F1 & CoNLL F1 \\
\midrule
0 & 34.4 & 88.3 & 49.5 & 45.5 & 91.3 & 60.7 & 52.7 & 17.0 & 25.8 & 30.4 & 29.4 & 29.9 & 45.3 \\
1 & 100.0 & 83.2 & 90.8 & 100.0 & 35.6 & 52.6 & 21.1 & 68.5 & 32.3 & 99.5 & 32.1 & 48.5 & 58.6 \\
2 & 95.8 & 83.0 & 89.0 & 95.4 & 40.3 & 56.6 & 27.4 & 57.8 & 37.2 & 93.4 & 33.5 & 49.3 & 60.9 \\
3 & 76.3 & 83.1 & 79.6 & 75.0 & 61.1 & 67.4 & 46.9 & 36.7 & 41.2 & 67.8 & 39.3 & 49.7 & 62.7 \\
4 & 57.7 & 89.3 & 70.1 & 58.9 & 85.5 & 69.7 & 61.5 & 27.8 & 38.3 & 47.7 & 48.2 & 47.9 & 59.4 \\
5 & 87.9 & 82.0 & 84.8 & 86.0 & 44.8 & 58.9 & 32.5 & 43.1 & 37.1 & 81.9 & 32.0 & 46.0 & 60.3 \\
6 & 68.9 & 86.6 & 76.7 & 68.0 & 74.6 & 71.2 & 56.1 & 33.0 & 41.6 & 59.1 & 46.6 & 52.1 & 63.2 \\
7 & 76.6 & 83.9 & 80.1 & 75.1 & 63.9 & 69.1 & 50.0 & 38.5 & 43.5 & 67.8 & 42.8 & 52.5 & 64.2 \\
8 & 72.5 & 86.0 & 78.7 & 71.3 & 71.6 & 71.4 & 55.8 & 36.3 & 44.0 & 63.1 & 47.3 & 54.1 & 64.7 \\
9 & 59.3 & 88.8 & 71.1 & 59.6 & 83.4 & 69.5 & 61.9 & 29.0 & 39.5 & 48.6 & 47.5 & 48.1 & 60.0 \\
10 & 88.5 & 83.7 & 86.0 & 87.5 & 51.0 & 64.4 & 39.3 & 49.1 & 43.7 & 83.2 & 38.5 & 52.6 & 64.7 \\
11 & 77.3 & 84.1 & 80.6 & 75.7 & 63.4 & 69.0 & 48.5 & 37.8 & 42.5 & 68.4 & 42.6 & 52.5 & 64.0 \\
12 & 64.9 & 82.9 & 72.8 & 64.3 & 71.8 & 67.8 & 53.6 & 30.7 & 39.0 & 54.4 & 41.8 & 47.3 & 59.9 \\
13 & 84.3 & 84.0 & 84.2 & 83.0 & 56.2 & 67.0 & 43.0 & 43.6 & 43.3 & 77.5 & 40.5 & 53.2 & 64.8 \\
14 & 72.6 & 85.0 & 78.3 & 71.4 & 69.3 & 70.4 & 53.3 & 35.6 & 42.7 & 63.2 & 44.8 & 52.4 & 63.8 \\
15 & 76.9 & 84.8 & 80.6 & 75.7 & 64.3 & 69.5 & 49.6 & 37.7 & 42.8 & 68.3 & 42.9 & 52.7 & 64.3 \\
\bottomrule
\end{tabular}
\end{table*}

